Embodied Question Answering

We present a new AI task -- Embodied Question Answering (EmbodiedQA) -- where an agent is spawned at a random location in a 3D environment and asked a question ("What color is the car?"). In order to answer, the agent must first intelligently navigate to explore the environment, gather information through first-person (egocentric) vision, and then answer the question ("orange"). This challenging task requires a range of AI skills -- active perception, language understanding, goal-driven navigation, commonsense reasoning, and grounding of language into actions. In this work, we develop the environments, end-to-end-trained reinforcement learning agents, and evaluation protocols for EmbodiedQA.

==> sections/main/evaluation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{\sectionReduceTop}
%\section{Evaluating \eqa Agents}
\section{Evaluation Protocols}
\label{sec:evaluation}
%\vspace{\sectionReduceBot}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The ultimate goal of an \eqa agent is to answer questions accurately. However, 
it is important to disentangle success/failure at the intermediate task of navigation 
from the ultimate downstream task of question answering. 

%this task is difficult and failures may be due to deficiencies in navigation or
%question answering. As such, we present metrics evaluating both agents' final answers
%and their intermediate navigation. 

\xhdr{Question Answering Accuracy.} 
Our agent (and all baselines discussed next) produce a probability distribution over $172$ possible answers 
(colors, rooms, objects). We report the mean rank ($\mathbf{MR}$) of the ground-truth answer in 
the answer list sorted by the agent's beliefs, where the mean is computed over all \texttt{test} questions and environments. 
%Since all answers are unambiguous and 1-2 word phrases, we can use classification\verify{/retrieval} metrics to 
%compute answering accuracy. Specifically, we report \verify{top-$\{1,3,5\}$ accuracy, mean rank, 
%and mean reciprocal rank of the ground-truth answer 
%in the answer list sorted by the agent's confidence.}
%As each question type depends on a different skill set, we 
%breakdown evaluation by question type: reporting 

\xhdr{Navigation Accuracy.} 
%Most questions do not have a unique or natural `correct' navigation required to answer them.  
%-- there may be multiple paths with varying degree of exploration that may let the agent accumulate visual 
%One virtue of questions in \eqads v1.0 is that there is a natural single target queried object. 
%Many questions depend on either single objects or multiple objects withina single room in the environments. 
%For these questions, we can measure navigational success 
%in terms of an agents progress towards these targets. 
We evaluate navigation performance on \eqads v1 by reporting the 
%the average across episodes for the number of actions $\left(\mathbf{{\mbox{\textbf{T}}}}\right)$, 
distance to the target object at navigation termination $\left(\mathbf{d_T}\right)$, 
change in distance to target from initial to final position $\left(\mathbf{{d_\Delta}}\right)$, 
and the smallest distance to the target at any point in the episode $\left(\mathbf{{d_{min}}}\right)$. 
\verify{All distances are measured in meters along the shortest path to the target.} 
%As distance can be hard to relate to question answering success, 
We also record the percentage of questions for which an agent either 
terminates in $\left(\mathbf{\%r_T}\right)$ 
or ever enters $\left(\mathbf{\%r_{\dlsh}}\right)$ the room containing the target object(s). 
Finally, we also report the percent of episodes in which agents choose to terminate navigation and 
answer before reaching the maximum episode length $\left(\mathbf{\%stop}\right)$.

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth,clip=true, trim=10px 10px 50px 50px]{figures/top_down_visualizations.pdf} \\
\label{fig:top-down-viz}
\caption{Top-down visualizations of the path taken by the agent.}
\end{figure}

% %stopped runs
% ended in correct room
% mean #actions
% terminal distance
% terminal - initial distance


% closest pass to target
% entered room

\begin{comment}


\ad{
    Intuitively, an \eqafull agent should be good at
    both question-guided navigation as well as accurate answer prediction.
    We evaluate our models on seen and unseen environments as well as seen
    and unseen questions.
}

\ad{
    \textbf{Navigation}. Inspired by prior work in goal-driven navigation~\cite{khosla_cvpr14,brahmbhatt_cvpr17,
    zhu2017target,gupta_cvpr17}, we develop the following metrics.
    \textbf{Partial success rate\footnote{needs a better name?}.} \devi{Like we discussed, this is an 
    experiment set up. Not an evaluation metric.So should include it in the list of ablations / 
    baselines / upper bounds we evaluate. And agree, should rename. Then don't need to mention 
    various values of $t_-$ in description of metrics that follow.} We initialize the agent
    $t_-$ steps before the target along the human navigation path, and compute the fraction
    of times the agent successfully reaches its target. We evaluate this for $t_- = 10, 50, 100, \infty$,
    where $t_- = \infty$ implies initializing at the human spawn location.
    \textbf{Average no. of steps.} Average no. of steps taken to reach the target
    in successful runs, for $t_- = 10, 50, 100, \infty$.
    \textbf{Expected no. of steps.} If $s_{t_-}$ is the partial success rate,
    $L_{t_-}$ the average no. of steps for successful trials and $L_\text{max}$ the maximum
    no. of steps, then $s_{t_-} \times L_{t_-} + (1-s_{t_-}) \times L_{\text{max}}$,
    for $t_- = 10, 50, 100, \infty$.
    Note that for $t_- = \infty$, these are the same metrics as in~\cite{brahmbhatt_cvpr17}.
}

\devi{Should we analyze something about the shape of the path the agent takes? How smooth it 
is? Relative to human paths say? Should we count how often it visits the same spot? That might 
not happen very often though. Can measure how often it visits the same room after it left it. Should 
we measure how distance to target (when defined) goes down as number of steps increase? Does 
the model make steady progress all along, or is bouncing around for a while and then starts 
making progress? Something in between? Again, can compare to humans. This can actually be a 
good use of human data. If we think of various properties / stats to measure for machine paths, we 
can compare to same stats for human paths (and shortest path). Are there certain rooms the bot 
tends to visit? Are there certain rooms the bot never gets to? Where is the bot present usually 
relative to the center of the home say? Usually towards the interior? Or towards the exterior? Or 
does it tend to get trapped in a local region around where it is spawned? Does the behavior vary 
based on which room it is spawned in? If spawned in a bathroom, does it get stuck more often 
than in the living room say? Does the agent always go all over the house irrespective of how far it 
was from the target? We could cluster paths in some reasonable way to visualize clusters of 
behaviors these agents tend to have. Do we ever ask multiple questions about the same object? 
We could at test time for some small number of cases. If there are multiple questions that all 
require the same navigation (e.g., what color is the chair in the dining room? and what is on the 
chair in the dining room?) but different VQA processing, does our model realize that? Probably 
not. But is it worth analyzing the extent to which the paths taken are similar? Some of this is 
similar to the kind of analysis Aishwarya did for her EMNLP paper that analyze the behavior of 
VQA models. Would be fun to do that for these agents! Maybe even think of adjectives to describe 
them: Are they focussed? Or do they bounce off of walls? Do they have clarity of thought? :) Not 
sure if all this fits in ``Evaluation'' which is before Approach, or in ``Analysis'' after we present the 
approach and results. Latter makes more sense so we can get to the approach soon enough.}

\devi{We will need a way to visualize the path the agent took on a top-down view of the 
environment, right? Will that be easy-ish to do?}

\ad{
    \textbf{Question answering}.
    We break down answering accuracy by question type, and report top-$\{1,3,5\}$
    accuracies.
} \devi{yes! I've been wanting a way to soften this metric because chances are the model is never 
going to get any answer right! Ok, maybe that's a bit extreme. But still. This is a good idea (I now 
remember discussing this earlier).}

\end{comment}
